On Compensation Primitives as Adaptable Processes

We compare mechanisms for compensation handling and dynamic update in calculi for concurrency. These mechanisms are increasingly relevant in the specification of reliable communicating systems. Compensations and updates are intuitively similar: both specify how the behavior of a concurrent system changes at runtime in response to an exceptional event. However, calculi with compensations and updates are technically quite different. We investigate the relative expressiveness of these calculi: we develop encodings of core process languages with compensations into a calculus of adaptable processes developed in prior work. Our encodings shed light on the (intricate) semantics of compensation handling and its key constructs. They also enable the transference of existing verification and reasoning techniques for adaptable processes to core languages with compensation handling.

==> eptcsdata.tex <==
\providecommand{\firstpage}{16}
\providecommand{\publicationstatus}{S. Crafa and D. Gebler (Eds.): Combined Workshop on Expressiveness in\\ Concurrency and Structural Operational Semantics (EXPRESS/SOS 2015)\\
EPTCS 190, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.190.2}{10.4204/EPTCS.190.2}}

